NovaQ: Improving Quantum Program Testing through Diversity-Guided Test Case Generation

Quantum programs are designed to run on quantum computers, leveraging quantum circuits to solve problems that are intractable for classical machines. As quantum computing advances, ensuring the reliability of quantum programs has become increasingly important. This paper introduces NovaQ, a diversity-guided testing framework for quantum programs. NovaQ combines a distribution-based test case generator with a novelty-driven evaluation module. The generator produces diverse quantum state inputs by mutating circuit parameters, while the evaluator quantifies behavioral novelty based on internal circuit state metrics, including magnitude, phase, and entanglement. By selecting inputs that map to infrequently covered regions in the metric space, NovaQ effectively explores under-tested program behaviors. We evaluate NovaQ on quantum programs of varying sizes and complexities. Experimental results show that NovaQ consistently achieves higher test input diversity and detects more bugs than existing baseline approaches.

==> IEEE-conference-template-062824/note.tex <==
ASE 2025 NIER Paper #51 Reviews and Comments
===========================================================================
Paper #51 NovaQ: Improving Quantum Program Testing through Diversity-Guided
Test Case Generation


Review #51A
===========================================================================

Overall merit
-------------
3. Weak accept

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The paper presents NovaQ, a diversity driven approach for testing quantum programs. The testing approach has two main components: a distribution-based test generation and a novelty-driven evaluator. The authors built the test generator based on a controlled mutation of sampled distributions. For the test evaluator, the paper gives a score for the quantum state vectors based on the metrics such as magnitude, phase, and entanglement. The results across circuits of varying sizes show that NovaQ is able to generate diverse test cases and detect bugs in quantum programs.

Comments for authors
--------------------
# Strengths
* The paper focuses on an important and timely problem of quantum software systems.
* The paper is well structured and clearly written. 
* The results are promising and demonstrate the effectiveness of the proposed approach.

# Weaknesses
* Only one type of quantum program is used for bug detection.
* More baselines could be included to compare the effectiveness of NovaQ over coverage-based testing methods. 
* The significance of the results could be further discussed, in relation to existing testing methods.


The paper is well written and structured. The methodology is clearly described with adequate discussion on the related works. The paper also focuses on a novel approach for diversity-driven testing of quantum programs. The combination of a distribution-based test generation and a novelty-driven evaluator is a promising direction for testing quantum programs. 

I find the use of quantum state metrics such as magnitude, phase, and entanglement to evaluate the diversity of test cases most interesting in the paper. The novelty score makes sense and is combined with the iterative selection process. While the technique is in early stage, the evaluation shows promise for certain types of quantum programs.

The paper could be improved by including more diverse quantum programs for bug detection, as well as additional baselines to compare the effectiveness of NovaQ against existing coverage-based testing methods. Thus, the generalizability is not clearly demonstrated. The significance of the results could also be discussed in more detail, especially in relation to existing testing methods.



Review #51B
===========================================================================

Overall merit
-------------
4. Accept

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
The paper introduces NovaQ, a novel diversity-guided test generation technique for quantum programs. The approach comprises two main components: a distribution-based test input generator and a novelty-driven evaluator. By iteratively generating and selecting inputs that target underexplored regions of the testing space, NovaQ enhances test coverage. Experimental results indicate that the technique outperforms the baseline in both test input diversity and bug detection effectiveness.

Comments for authors
--------------------
Significance: The paper addresses a timely and highly relevant problem in quantum software engineering. It shows a great potential for future impact as quantum computing grows more complex. 

Novelty:
While diversity-based test generation is established in classical software testing, the application of guided mutation and novelty evaluation to quantum states is a novel and compelling direction.

Soundness:
The core idea is logically sound, and the preliminary results are promising. However, the paper would benefit from a more detailed description of the experimental setup and methodology. Additionally, since fault injection was performed manually, including information about the types and nature of the faults would enhance the clarity and credibility of the evaluation.

Presentation:
The paper is clearly written and well-structured. That said, certain sections, including the research methodology, could be improved by providing additional detail.



Review #51C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
1. No familiarity

Paper summary
-------------
Testing of quantum programs is challenging due to the nondeterministic and
probabilistic nature of quantum behavior along with the complexities of the
quantum circuits on which these programs run. This paper presents NovaQ as a
new framework for generating tests for quantum programs. NovaQ generates test
inputs that are gate parameters, sampled from a Gaussian distribution, applied
to an initial quantum circuit to execute. It also uses a mutator to perturb the
mean and variance of the parameter distribution as it iteratively generates
more tests. NovaQ also relies on novelty score computed based on a circuit's
internal state, meant to quantify the behavioral diversity and help guide test
generation towards exploring more diverse circuit behaviors. An evaluation of
NovaQ on a set of quantum programs shows that it can generate tests that
exhibit more diverse behavior and expose more bugs than prior test generation
approaches.

Comments for authors
--------------------
Quantum programs are indeed a new, still unexplored domain, so exploring
testing in this domain is interesting. I do appreciate the paper describing the
basics of quantum programs and what it means to do "testing" in this domain,
namely needing to set gate parameters for the quantum circuits. I like how the
paper tries to transplant traditional testing concepts in sampling and mutating
inputs to generate the actual tests as well as developing metrics to evaluate
the quality of the tests.

The main concern I have is whether the proposed novelty score is truly
indicative of diverse circuit behaviors that are useful indicators of exploring
the "space" of programs and finding bugs. My understanding is that the novelty
score is brand new, so I am not sure whether there is a strong correlation
between this score and fault-detection capability. Half of the evaluation seems
to be focused on this new metric, especially when compared against other
baselines, so it is important to consider how important this metric is. I do
like how the evaluation does also consider actual fault-detection capability
through injected faults when comparing against baselines.

The paper should also comment on how the approach can apply more broadly, when
removing some of the restrictions of the evaluation such as circuit size or
complexity. Basically, what would be the main limitations that NovaQ might
suffer from if applied to a broader range of quantum programs, like briefly
mentioned as future work in the Conclusions. I think such discussion is
warranted to better understand the proposed approach and its potential
generalizability.



Comment @A1 by Reviewer B
---------------------------------------------------------------------------
****Meta-Review****

Testing quantum programs presents unique challenges due to their nondeterministic and probabilistic behaviour, as well as the inherent complexity of quantum circuits. This paper introduces NovaQ, a diversity-guided test generation framework designed to address these challenges. The approach combines a distribution-based test input generator with a novelty-driven evaluator that selects inputs targeting underexplored regions of the program’s behaviour space. Experimental results show that NovaQ produces test inputs that exhibit higher behavioural diversity and uncover more bugs compared to existing approaches.

Comments for Authors:
All reviewers agree that the topic is relevant and timely in the domain of quantum software engineering. The integration of a distribution-based generator with a novelty-guided evaluator is recognised as a promising direction. The paper is well-structured, clearly written, and the methodology is easy to follow. While the technique is in an early stage, the evaluation demonstrates its potential for certain classes of quantum programs. Based on these strengths, all reviewers accepted this paper for publication. 

Several concerns raised by reviewers that could further strengthen the work are: 
1. One concern is the validation of the novelty score. Since it is a new metric, it would be valuable to explore its correlation with fault-detection capability to better establish its effectiveness. 
2. The generalisability of NovaQ could be improved by testing across a broader set of quantum programs and by including additional baselines, particularly coverage-based approaches. 
3. As fault injection was performed manually, the paper would benefit from a clearer description of the types and nature of the injected faults to improve the transparency and reproducibility of the evaluation.

ASE 2025 NIER 论文 #51 评审意见
论文 #51 NovaQ: Improving Quantum Program Testing through Diversity-Guided Test Case Generation
（通过多样性引导的测试用例生成提升量子程序测试）

评审 #51A
整体评价
3. 弱接收（Weak accept）

评审人专业背景
2. 有一定了解（Some familiarity）

论文摘要
本文提出了 NovaQ，一种面向量子程序的多样性驱动测试方法。该测试方法主要包含两个部分：基于分布的测试生成器，以及基于新颖度驱动的评估器。作者基于对采样分布的受控变异构建了测试生成器。在测试评估器部分，论文根据幅度（magnitude）、相位（phase）和纠缠度（entanglement）等指标，为量子态向量打分。跨不同规模电路的结果显示，NovaQ 能够生成多样化的测试用例，并在量子程序中发现缺陷。

给作者的意见
优点：

本文关注量子软件系统中一个重要且及时的问题。

论文结构合理、表达清晰。

结果具有前景，展示了所提方法的有效性。

不足：

缺陷检测仅使用了一种类型的量子程序。

可以增加更多基线方法，与 NovaQ 在覆盖率驱动的测试方法上进行比较。

结果的重要性可以进一步结合现有测试方法进行讨论。

总体而言，论文写作和结构良好，方法论描述清晰，并对相关工作进行了充分讨论。本文关注于一种新颖的量子程序多样性驱动测试方法，将基于分布的测试生成与新颖度驱动的评估相结合，是量子程序测试的一个有前景方向。

我认为本文中使用量子态的幅度、相位和纠缠度来评估测试用例多样性是最有趣的部分。新颖度评分合理，并与迭代选择过程相结合。虽然技术尚处于早期阶段，但评估结果在特定类型量子程序上显示了潜力。

改进建议包括：在缺陷检测中引入更多类型的量子程序，以及更多基线方法来与现有覆盖率驱动测试进行比较。此外，应更详细地讨论结果的重要性，尤其是与现有测试方法的关系。

评审 #51B
整体评价
4. 接收（Accept）

评审人专业背景
3. 较为熟悉（Knowledgeable）

论文摘要
本文介绍了 NovaQ，一种新颖的多样性引导量子程序测试生成技术。该方法包括两个主要部分：基于分布的测试输入生成器，以及基于新颖度驱动的评估器。通过迭代生成并选择针对测试空间中未充分探索区域的输入，NovaQ 提升了测试覆盖率。实验结果表明，该技术在测试输入多样性和缺陷检测有效性方面均优于基线方法。

给作者的意见

意义（Significance）： 本文聚焦于量子软件工程中一个及时且高度相关的问题。随着量子计算日益复杂，该方法具有巨大的未来影响潜力。

新颖性（Novelty）： 尽管多样性驱动的测试生成在经典软件测试中已有研究，但将引导变异与新颖度评估应用于量子态是一个新颖且引人注目的方向。

合理性（Soundness）： 核心思想在逻辑上是合理的，初步结果令人鼓舞。然而，论文若能更详细地描述实验设置与方法，将更具说服力。此外，由于缺陷注入是手动完成的，若能说明注入缺陷的类型与性质，将有助于提升评估的清晰度与可信度。

表达（Presentation）： 论文结构清晰，写作流畅。但包括研究方法在内的部分章节仍可通过增加细节来改进。

评审 #51C
整体评价
2. 弱拒绝（Weak reject）

评审人专业背景

不熟悉（No familiarity）

论文摘要
由于量子行为的非确定性与概率特性，以及量子电路本身的复杂性，测试量子程序面临巨大挑战。本文提出 NovaQ 这一新框架用于生成量子程序的测试用例。NovaQ 生成的测试输入是门参数，这些参数从高斯分布采样，并应用于初始量子电路执行。它还使用变异器在迭代生成测试过程中扰动参数分布的均值和方差。此外，NovaQ 基于电路的内部状态计算新颖度评分，以量化行为多样性并引导测试生成探索更多样化的电路行为。对一组量子程序的评估表明，NovaQ 能够生成行为更为多样的测试，并比以往的测试生成方法发现更多缺陷。

给作者的意见
量子程序确实是一个新颖且尚未充分探索的领域，在这一领域开展测试研究是有价值的。我赞赏本文解释了量子程序的基础知识，以及在该领域进行“测试”的含义——即需要为量子电路设定门参数。我喜欢本文将传统测试中的采样与变异概念移植到量子程序输入生成中，并提出评估测试质量的指标。

我主要的担忧是，所提出的新颖度评分是否真的能有效反映对电路行为多样性的有用探索，以及其与缺陷检测能力的关联程度。我的理解是该评分是全新的，因此尚不清楚其与缺陷检测能力之间是否存在强相关性。论文有一半的评估似乎集中在这一新指标上，尤其是与其他基线的比较，因此应重视其重要性。同时，我也认可本文在比较基线时考虑了通过缺陷注入来评估实际缺陷检测能力。

此外，论文还应讨论该方法在更广泛应用场景下的适用性，比如在取消评估中电路规模或复杂度等限制的情况下。基本上，需要明确 NovaQ 在更广泛类型的量子程序上的潜在限制，如在结论中提到的未来工作。这类讨论有助于更好地理解所提方法及其可推广性。

评审人 B 的元评（Meta-Review）
测试量子程序具有独特挑战，因为其行为具有非确定性和概率性，同时量子电路本身也非常复杂。本文提出的 NovaQ 是一个多样性引导的测试生成框架，旨在应对这些挑战。该方法将基于分布的测试输入生成器与新颖度驱动的评估器相结合，从而选择针对程序行为空间中未充分探索区域的输入。实验结果表明，NovaQ 生成的测试输入在行为多样性上更高，并能比现有方法发现更多缺陷。

给作者的综合意见：
所有评审人一致认为，该主题在量子软件工程领域具有相关性与及时性。将基于分布的生成器与新颖度引导的评估器相结合被认为是一个有前景的方向。论文结构合理，写作清晰，方法易于理解。尽管该技术仍处于早期阶段，但评估显示了其在特定类别量子程序中的潜力。基于这些优点，所有评审人均建议接收该论文。

为进一步加强工作，评审人提出了以下几点建议：

验证新颖度评分。由于该指标是全新的，建议探索其与缺陷检测能力之间的相关性，以更好地确立其有效性。

提升 NovaQ 的可推广性，可通过在更广泛的量子程序上进行测试，并引入更多基线方法（尤其是覆盖率驱动方法）进行比较。

由于缺陷注入是手动进行的，建议更清楚地描述注入缺陷的类型与性质，以提升评估的透明度和可复现性。



==> IEEE-conference-template-062824/xiugaidagang.tex <==



在RQ3.中加一句，Bug的手动注入方法本文所使用的含有bug的被测程序是在正常的量子软件算法（如grover算法）所表示的量子电路中用至少一个随机的门去替换对应位置的门。根据Definition 2.的定义，对于给定的testcase作为被测程序的输入，the output probability和预期不一样，就可以说明被测程序存在bug。

加入adder或者PE和qft测试结果  以-05为例

在RQ3中解释，testcase多样性越高，测出的bug程序数量就越多，这是因为对于一个量子程序来说存在很多分支，根据Definition 2.定义，bug可能存在于任何一个分支中，testcase种类越多，能测试的分支组合就越多，越容易找出bug。
